On the pragmatism of using binary classifiers over data intensive neural network classifiers for detection of COVID-19 from voice

Lately, there has been a global effort by multiple research groups to detect COVID-19 from voice. Different researchers use different kinds of information from the voice signal to achieve this. Various types of phonated sounds and the sound of cough and breath have all been used with varying degree of success in automated voice-based COVID-19 detection apps. In this paper, we show that detecting COVID-19 from voice does not require custom-made non-standard features or complicated neural network classifiers rather it can be successfully done with just standard features and simple binary classifiers. In fact, we show that the latter is not only more accurate and interpretable but also more computationally efficient in that they can be run locally on small devices. We demonstrate this on a human-curated dataset of over 1000 subjects, collected and calibrated in clinical settings.

==> ICASSP - Paper On Pragmatism COVID-19/expt.backup.tex <==
\section{Data and Experiments} \vspace{-2mm} 
\label{sec:experiments}

\subsection{Dataset and its description}
A key challenge in many of the previous studies was the data -- data that were trustworthy and medically reliable were generally small, while those that were collected at large scale were unreliable (being mostly self-reported) leading to unreliable results.  To address this issue, we require a dataset that is both reasonably large, and reliably annotated.
We used a dataset collected under clinical supervision and curated by Merlin Inc., a private firm in Chile. The subjects usually have symptoms of coughing, sneezing, breathing difficulties etc. So these related symptoms were also recorded along with the voice to account for symptomatic and asymtomatic COVID-19 diagnosis. The COVID positive or negative label was indicated by the subject's lab-certified test results. Additionally metadata also contained information about preexisting conditions such as smoking preference, asthma and detailed comments about the speakers health during the dataset generation. The data samples were recorded over a smartphone, and sampled at 8khz.  

The dataset consists of recordings from 421 covid-positive 989 covid-negative unique subjects. Subjects were asked to record themselves saying the elongated vowels /AH/, /UW/ and /IY/, and speaking the Spanish alphabet (a-z), counting from 1-20 (in Spanish) and producing coughs. 
%The voice recordings of a-z were segmented into vowels of /aaa/ /ee/ /oo/ based on the phonemes. 
To eliminate external influences, subjects were recorded in a quiet room environment.  
%So the dataset has a sampling rate of 8 khz as the microphone bandwidth. 
%The following dataset provides information about the statistics of different metrics in the dataset. 
The total duration of the covid-positive recordings is 17.5 hours, and for covid-negative recordings is 20.5 hours with over 37 hours of total data.

The careful curation of data also enabled us to compile additional statistics that are likely to be relevant to Covid-19. 

Figure \ref{fig:symptoms} shows a chart of symptoms for covid-positive and covid-negative subjects.
\begin{figure}[h]
\centering
\includegraphics[width=8.5cm, height=4cm]{symptoms_0_plot_2.png}
\includegraphics[width=8.5cm, height=4cm]{symptoms_1_plot_2.png}
\caption{The top figures shows the distribution of symptoms in COVID-19 positive patients and the lower figure is the distribution of symptoms in COVID-19 negative individuals (breath-diff stands for breathing difficulty). The rows represents each symptom whereas the column represents the frequency of occurrence of a symptom which are marked by dots}\label{fig:symptoms}
\end{figure}

The occurrence of Covid (and the symptoms arising from it) is also reportedly related to the age and gender of the subjects. Moreover, its symptoms  

\subsection{Experiments}

We perform numerous experiments for the detection of COVID where the input is only the voice signal. In all experiments, the speakers in the training set were separate from those in the test set to ensure that the models do not inadvertently simply capture speaker identity. Thus, we split the data in $k$ fold cross-validation sets based on speaker identity.
%ies by first selecting the speaker and keeping all recordings corresponding to that speaker in the same set. This type of split which is different from research papers published will ensure that there is no bias and we will have an unseen speaker in the testing set due to the experimental design, thereby rendering speaker-id identifying features useless. 

We run various classifiers on our data such as RandomForest (RF), Support Vector Machines (SVMs) with Radial Basis Function and Logistic Regression (LR). We analysed all the spectral features on each of these classifiers including combination of features like Ovec and Custom. The RandomForest runs on $k$ fold equal to 3, 5 and 10. We run grid search on all these classifiers to find the best parameters, particularly experimenting with $\gamma$. We report the performance in the  Section \ref{sec:results}.

\section{Results and Discussion}
\label{sec:results}
From the dataset consisting of a total of 1410 speakers (or 8460 audio recordings), the entire metadata was received for a total of 815 speakers, out of which there were 296 males and 519 females. \vspace{-2mm} 
\subsection{Age based Analysis}
We have broadly categorized the ages into four groups, including the ones whose age was missing, shown in Table \ref{tab:gender_table}.
\begin{itemize}[leftmargin=*] \itemsep0em
    \item Group 1 : age $<=$ 30 years
    \item Group 2 : 30 $<$ age $<=$ 40 years
    \item Group 3 : 40 years $<$ age
    \item Group 4 : Age was missing
\end{itemize}
For patients with age $>$ 40, our classifier is capable of recognizing COVID-19 patients accurately 65\% of the times whereas those with age $<$ 30, classifier is capable of accurately detecting 56\% of the times. 
\begin{table}[h]
    \centering
    \begin{tabular}{|c|c|c|c|c|}
        \hline 
        \textbf{Gender} & \textbf{Group1} & \textbf{Group2} & \textbf{Group3} & \textbf{Group4} \\
        \hline \hline
            Male & 65 & 80 & 80 & 71\\
            Female & 127 & 129 & 145 & 115 \\
            \hline
    \end{tabular}
    \caption{Gender based age analysis}
    \label{tab:gender_table}
        \vspace{-2mm}
\end{table}
The classifier is more reliably able to detect COVID-19 in case of females over males. 
% \begin{figure}[h]
% \centering
% \includegraphics[width=8cm, height=2.5cm]{images/age_dist_0.JPG}
% \includegraphics[width=8cm, height=2.5cm]{images/age_dist_1.JPG}
% \caption{The top figure is the age distribution for Covid positive patients and the lower figure is the age distribution for Covid negative individuals.}
%     \vspace{-2mm}
% \end{figure}





We find Sore-throat is present in most of COVID-19 cases where we are able to detect COVID-19 in 57\% of the cases. When sneeze is present, the classifier is capable of detecting COVID-19 in 47\% of the cases. When cough is a known  symptom for the speaker, then our classifier detects COVID-19 in 73\% of the cases.  \vspace{-2mm} 

\subsection{Smokers and People with Asthma}
Having a previous history of asthma or smoking might put people at a higher risk of COVID \cite{asthma}. We received data where people had a history of asthma and/or were smokers. Table \ref{tab:asthma_table} shows the statistics in our data. Our experimental results indicate asthama is more correlated to COVID-19 than smoking.  
For the patients with COVID-19 and smoking habit, our classifier is accurate by detecting COVID-19 in 66 percent of cases whereas those with COVID-19 and asthama cases we are able to detect COVID-19 accurately in 80 percent of the cases. 

\begin{table}[h]
    \centering
    \begin{tabular}{c|c|c}
        \textbf{Gender} & \textbf{Has Asthma} & \textbf{Is Smoker} \\
        \hline \hline
            Male & 12 & 95\\
            Female & 38 & 139
    \end{tabular}
    \caption{Gender based asthma and smoker statistics}
        \vspace{-4mm}
    \label{tab:asthma_table}
\end{table}


\subsection{Difference in days of diagnosis and data collection }  % \vspace{-2mm} 
The data collection process introduces a delay between the COVID onset and when the voice sample was recorded. Each speaker is labelled for the day they got diagnosed and the day they recorded their data.  Table \ref{tab:diagnosis_table} shows number of people distribution depending on when they were diagnosed (eg. 1 week ago, between 1-2 weeks or greater than 2 weeks) 

\begin{table}[h]
\centering
    \begin{tabular}{ |c|c| } 
         \hline
         \textbf{Diagnosis Day Range} & \textbf{Number of People} \\
         \hline \hline
         Diagnosis day $<=$ 7 days & 95 \\ 
         \hline
         7 days $<$ Diagnosis day $<=$ 14 days & 209 \\ 
         \hline
         Diagnosis day $>$ 14 days & 159 \\ 
         \hline
         Diagnosis day not known & 37 \\
         \hline
    \end{tabular}
    \caption{Difference between Diagnosis Day and Data collection day}
    \vspace{-4mm}
    \label{tab:diagnosis_table}
\end{table}

In general, we find that COVID-19 can be more reliably detected for patients whose voice samples have been collected within 14 days of diagnosis, than for those whose samples were collected after this period.



% For the detection of COVID-19 depending on the amount of diagnosis days, we find that COVID-19 can be reliably detected for patients which are less than 14 days and the degree of correlation for patients with greater than 14 days for diagnosis in the voice samples reduces. 

%Table 1 shows the confusion matrix of the related labels. 


% Confusion matrix


% We split the data into $k$ fold cross validation sets based on the speaker identities to avoid bias and have unseen speaker in the test process in the experimental design. 


%Finally, we use a deep neural network model, in an \textit{autoencoder} architecture using CNN, to extract learned features from the COVID dataset and then use those learned features in an MLP classification network. The details of the model are explained in the Experiment section. 

% Features which are present from pase features. Doesnt have direct correlation with noun capacity. Vocal tract of speech production mechanism 

% Not directly correlated feature in the detection pipeline. 
% Compare the spectrogram, pase and mfcc features --> reason why it is not 

% Randomforest 
% and CNN comparable results as the Randomforest 








% \subsection{Experiments using the different folds}
% We perform K fold cross validation on the dataset. To 
% In order to make full usage of the dataset, we have done the K-folds setting. To do so, we divide the dataset according to the speakers into K-fold for training and testing. The speakers in the test set is not seen in the training set. 
%We perform grid search 


% \section{Results and Discussion}
% 

\begin{table}[h]
    \centering
    \resizebox{1.0\columnwidth}{!}{
    \begin{tabular}{|c|c|c|c|}
    \hline 
       \textbf{Classifier}  &  \textbf{Feature}  & \textbf{AUC} \\ 
       \hline \hline
        Random Forest & Ovec & 0.76 \\
        Random Forest & PANN & 0.78    \\
        Random Forest & vggish & 0.59   \\
        Random Forest & Open-L3 & 0.64   \\
        Random Forest & YAMNet & 0.72   \\
        Random Forest & Custom  Feat & 0.82  \\ 
        Random Forest & Ovec + Custom  Feat & 0.84  \\
        Random Forest & Ovec + Custom Feat + vggish & 0.82  \\
        Random Forest & Ovec + custom feature + YAMNet & 0.86  \\ 
        CNN & Spectrogram & 0.69   \\
        CNN & PASE & 0.73     \\ 
        \hline
    \end{tabular}
    }
    \caption{Results obtained on the full dataset set. Here Ovec refers to features obtained using OpenSMILE, PASE using PASE architecture, custom spectral feature. Random Forest classifier is robust and have improved performance in comparison to CNN based classifier}
    \label{tab:my_label}
        \vspace{-4mm}
\end{table}
\vspace{-2mm} 
\subsection{Audio type analysis}  
% vowel 
We analyze classifier performance according to the audio-type, to identify which type of recording is most suited to capture the voice signatures related to COVID-19. Our results indicate that vowel /IY/ and vowel /UW/ are better at detecting COVID-19 than other types of audio samples. Cough samples are also useful in detecting COVID-19. \vspace{-2mm} 
\subsection{Overall Classifier results} 
Table \ref{tab:my_label} proves our hypothesis that a binary classifier such as Random Forest can perform better for COVID-19 detection than CNN counterparts when faced with limited data. Our experiments have observed that Open-L3 features perform the same as vggish feature representations. Figure \ref{fig:Best} shows the best AUC score achieved of 0.94 and ROC score of 0.85 for the Random forest based classifier with Ovec and custom features on a trimmed down dataset where 20\% samples were heard to contain noise in the recordings. 

\begin{figure}[h]
\centering
\begin{subfigure}[b]{0.23\textwidth}\centering
\includegraphics[width=\textwidth,height=3cm]{roc_auc.png}
\end{subfigure}
\begin{subfigure}[b]{0.23\textwidth}\centering
\includegraphics[width=\textwidth,height=3cm]{prec_recall.png}
\end{subfigure}
 \hspace*{\fill}
\caption{AUC of 0.94 and  ROC of 0.85 is obtained using Random Forest based classifier with Ovec and custom feature vector}
\label{fig:Best}
\end{figure}


\section{Conclusion}
\label{sec:discuss}
Motivated by the urgent need to have alternative methods to augment the medical tests, we designed the experimental setup for the COVID-19 analysis using a wide variety of voice samples. Our analysis provided insights into the type of voice sample which would work best for detecting COVID-19 patients which is the \/eee\/ and \/ooo\/ sounds. Our COVID-19 dataset used in the study was acquired through self-recording using a smartphone application making acquistion feasible at large scale. The preliminary results imply a feasibility for the use of this globally accessible data collection for Sars-COV-2 detection although it doesn't replace RT-PCR or RAT tests.  Our results prove that using a binary classifiers such as Random Forest are more feasible to separate between COVID-19 vs non COVID-19 speakers over data intensive neural network classifiers. We find these binary classifiers to generate better and robust results given the limited amount of data available for analysis. 






%\vfill\pagebreak

% \section{REFERENCES}
% \label{sec:refs}

% List and number all bibliographical references at the end of the
% paper. The references can be numbered in alphabetic order or in
% order of appearance in the document. When referring to them in
% the text, type the corresponding reference number in square
% brackets as shown at the end of this sentence \cite{C2}. An
% additional final page (the fifth page, in most cases) is
% allowed, but must contain only references to the prior
% literature.

% References should be produced using the bibtex program from suitable
% BiBTeX files (here: strings, refs, manuals). The IEEEbib.bst bibliography
% style file from IEEE produces unsorted bibliography list.
% -------------------------------------------------------------------------
\bibliographystyle{IEEEbib}
\bibliography{strings,refs}

==> ICASSP - Paper On Pragmatism COVID-19/intro.tex <==
The COVID-19 pandemic no longer needs an introduction, having sickened -- and killed -- millions of people worldwide in just a few months \cite{worldometer}. One of the primary weapons on our arsenal to combat this pandemic is isolation -- identifying infected or potentially infected individuals, and isolating them, to prevent them from infecting others. Identifying such individuals requires tests, and testing capacity for Covid-19 remains inadequate, with often unacceptable wait times during which an individual may spread the infection \cite{cvdtesting}. Consequently the search remains ongoing for rapid tests that can be quickly dispensed with minimal logistical challenges. Voice-based testing has been identified as one such possibility \cite{cvdvoicedetector}.

COVID-19 primarily manifests as an illness of the respiratory tract \cite{asiaee2020voice}, although other organs too are affected. In symptomatic patients, it affects the lower and upper respiratory tract \cite{9414201_soham}. While, by the very widespread nature of the pandemic and the shortage of testing capacity, the actual number of infected people and fraction of this population that exhibited specific symptoms can never be known precisely, various reports suggest that between 60\% and 80\% of symptomatic patients develop a dry cough \cite{song2021confronting}, and roughly a third develop a wet cough \cite{song2021confronting}. A common symptom is respiratory distress , and fluid accumulation in the lungs is frequently reported even in early-stage patients \cite{suess2020gross}. 

Naturally, it is to be expected that these impairments will manifest in the patient's vocalizations -- both in the form of coughing and in changes to their voice.  COVID-19 affects the three stages in voice production: respiration, phonation and the underlying resonant system \cite{asiaee2020voice}. The reduced lung capacity affects exhalation, affecting the mechanisms for the sub-glottal pressure and disrupting normal phonation \cite{asiaee2020voice}. In a self-assesment study, COVID patients reported difficulty producing certain voiced sounds and noticed changes in their voice \cite{lechien2020features}. 

Consequently, a number of research groups around the world have initiated efforts on attempting to diagnose potential Covid infections from recordings of vocalizations \cite{9414530_soham,9414201_soham}. While most groups have focused on cough sounds \cite{brown2020exploring, imran2020ai4covid, bagad2020cough} as they are a frequent symptom of Covid-19, several groups have also considered other vocalizations, such as breathing sounds \cite{brown2020exploring,10.1145/3394486.3412865} extended vowels \cite{RitaSinghTalkCambridge:2020, pinkas2020sars,schuller2021covid}, and counts. Yet other teams have analyzed free-form speech such as those obtainable from YouTube recordings\cite{shukla2021covid}. The general consensus appears to be that cough sounds \cite{10.1145/3394486.3412865}, and possibly speech sounds do provide discriminative information about the presence of COVID-19 . 

Promising results have also been obtained by using estimates of vocal fold oscillations \cite{9414530_soham,9414201_soham}. In all of these efforts, researchers have ubiquitously used neural networks for classification. Neural networks however require larger amounts of data for robust training. In the case of COVID-19 many groups have mentioned the difficulty in getting properly curated data in sufficient amounts that are needed for neural network training. Data insufficiency has cast a doubt on the basic premise of whether voice samples can accurately be used to detect COVID-19 from voice.  The question that this paper explores is : if we use classifiers for which data sufficiency is not such a critical issue, would the detection of COVID-19 from voice be positively affected. If so, \textit{i.e.} if simpler and less data intensive classifiers were able to achieve good results for detecting COVID-19 from voice then we could exploit this to create much faster, more robust and more accurate and more portable COVID-19 detection applications. 

While the premise of this paper is simple, this exploration is nevertheless crucial given the difficulty in obtaining clinical data not only for COVID-19 but also for many other health conditions. In this paper, we explore several simple classifiers and compare and contrast them to neural network based classifiers using standard features available publicly for voice analysis/speech applications. The latter is a choice that has been deliberately made in order to avoid the extra effort of inventing new features in a time-critical pandemic situation. It brings out the value of confidently relying on time-tested features and classifiers for detecting novel entities from voice. It brings out the importance of doing this exercise first before presuming that the situation is complex and that it requires complex solutions. Sometimes complex challenges do have easy to implement and simple solutions. It is purpose of this paper to highlight this. 


The rest of the paper is organized as follows. In Section 2, we discuss the work that has been done for detecting COVID-19 from voice from multiple perspectives. In Section 3, we describe the features and classifiers that have been used in multiple settings and explored by us in this paper for bringing out our main points. Section 4 describes the our data and experiments. In the section 5, we present our conclusions. 


% [THIS FOLLOWING PARA NEEDS UPDATE]
% %However, in spite of the initial encouraging results, the gap to an actual diagnostic tool remains large. In multiple  of these studies both the ``positive'' and ``negative'' instances of Covid are selfreported, leading to uncertainty in the data itself. Other results have been obtained from more reliable data collected from hospitals; the data collected, however, are mostly restricted to coughs and breathing sounds. Variations in cough and breathing patterns arise from a variety of pathologies, not just Covid-19 \cite{holfinger20190459, boulding2016dysfunctional, koyama2019application}, and in the absence of additional information (not the least because clinical data are generally protected), it remains unclear how much of the results obtained are attributable to Covid, as opposed other primary causes.  Also, the (results reported on the) data generally lack crucial information. Covid symptoms progress rapidly, with fast, rather dramatic changes occurring over a short period of time, and the rate of progression may vary with subject. Consequently, covid-induced vocalization patterns too change rapidly -- the cough or speech patterns of a person two days into symptomatic presentations of their infection will generally be vastly different from those of a person five days, a week, or two weeks into the infection. These are particularly relevant concerns, given the relatively low (albeit significantly better than random) classification accuracies reported (we will briefly expand on the practical implications of the low accuracies towards the end of this paper). 

% performance is poor regardless of approach

% [MOVE ON]




% Symptoms are nonunique
% changes are rapid

% reasonle size cough and voice data in clinical settings.
% cough alone or voice provides info?
% time from test
% age, gender and other factors

% Also vreify the classifier and features.



% FInally, is this good.

% Whether people had mask on or not (this analysis can be performed on oct 17 only data - if time exists - one line can be written for this - easy analysis)




==> ICASSP - Paper On Pragmatism COVID-19/related_work.tex <==
It is by now well known that speech can carry the signatures of numerous ailments \cite{singh2021overview}. Specifically, any ailment that affects any portion of the vocal apparatus may be expected to leave its signatures in voice.  Covid-19, which affects the lungs and muscles among other things, falls in this category. Consequently, many researchers have developed voice based analyzers for the detection of Covid-19 \cite{elizalde2021covid,9414201_soham,bagad2020cough,schuller2021covid,imran2020ai4covid,despotovic2021detection}. So far, the research has focused on two aspects -- the collection and curation of reliable data in possibly non-clinical settings (e.g. crowd-sourced settings) and  the determination of which vocal sounds might be most discriminative for the detection of Covid-19. Examples include Chloe et.al \cite{brown2020exploring} who collect cough and breathing samples from people who self-report as being infected with Covid. Although their data set is relatively large, the correlation between the true Covid-19 status of the speaker and their reported status is weak, compared to fully clinically validated data. They run SVM and Logistic Regression classifiers with handcrafted spectral features, but the results are unreliable due to the  errors that can be inadvertently or deliberately introduced in the process of self-reporting, as mentioned above.

The study by \cite{pinkas2020sars} analyzes selected vowel sounds from speech recordings of counting (e.g. from 50 to 80), collected over celluar phones, using neural networks. It concludes that the sounds of counting, in particular, the /z/ sound, are useful for distinguishing Covid. \cite{asiaee2020voice} report results on data collected in clinical settings and discuss how various acoustic parameters of vowel sounds like /aa/ change between the infected and non-infected people. The parameters analyzed include fundamental frequency, jitter and shimmer, HNR etc.

The AI4Covid Application (described in \cite{imran2020ai4covid}) performs analysis on 70 samples from subjects who were positive for Covid-19 and 96 Covid-negative samples and reports an 89\% F-1 score for the detection of Covid-19. However, since the data size used is small, the authors do not perform cross-validation experiments.

The study in \cite{pinkas2020sars} performs analysis of 29 Covid-positive and 59 Covid-negative patients' data with the sounds /ah/, /z/ and  counting. Their model extracts a feature representation using a transformer RNN network architecture with an added  speaker dissimilarity loss. The final score for their model is obtained using a libSVM-based classifier, yielding an AUC of  0.78, obtained with a leave-one-out based cross-validation strategy, owing to the small dataset size.  \cite{bagad2020cough} performs analysis on a relatively large-scale dataset comprising 376 positive cough samples, and 663 negative cough samples. The analysis uses a ResNet-based CNN architecture for making a binary prediction (Covid vs non-COVID) and yields an AUC of 0.68 on their dataset. However, their method uses a relatively high portion (90\%) of the total data for training.


The Coswara dataset \cite{sharma2020coswara} comprises breathing, cough, vocalized sounds, which include the vowels /e/, /i/, /a/, and shallow and fast deep breathing sounds collected from  Covid positive and negative patients. They attempt to classify 9 sound categories, with features such as spectral contrast, MFCC, spectral roll-off, zero-crossing rate, spectral bandwidth, spectral flatness etc.,  and achieve an accuracy score of 66.74\% on their test set. The low accuracy presumably stems from the split of the (small amount of) data.

\cite{10.1145/3394486.3412865} collected cough and breath sounds from 7000 unique users, but with only 235 covid-positive samples. Using a combination of features, including standard ones such as duration, tempo, RMS energy, spectral centroids and Vggish based features,  the approach yields an AUC of 0.8 for COVID vs non-COVID classification.

In all cases, the  reported performance is often either poor or unreliable, due to the unavailability of a sufficiently large and reliable dataset. The research community has yet to work on a dataset of sufficient size, with a high number of both covid-positive and covid-negative speakers, would be sufficiently large to perform reliable k-fold cross-validation with a large-parameter neural network classifier. Our goal in this paper is to find the cusp where the need for large amounts of data is minimized while the classification accuracy is not compromised. For this, we explore standard less-data intensive classifiers to find the best balance of dataset size, features and classifiers, to achieve our goal.


% according to their paper cough performs the worst and counting is more useful , /z/ sound is also useful as per this paper



% Chloe et.al \cite{brown2020exploring} collect data through voice recordings on a mobile device.

==> ICASSP - Paper On Pragmatism COVID-19/relatedwork.backup.tex <==
Analysis of vocal sounds has been investigated for the detection of numerous diseases \cite{singh2021overview}. Recently many researchers have developed voice based analyzers for the detection of Covid-19 \cite{9414201_soham,bagad2020cough,schuller2021covid,imran2020ai4covid,despotovic2021detection}. So far, the research has focused on two aspects -- the collection and curation of reliable data in possibly non-clinical settings (e.g. crowsourced settings) and  the determination of which vocal sounds might be most discriminative for the detection of Covid-19. Examples include Chloe et.al \cite{brown2020exploring} who collect cough and breathing samples from people who self-report as being infected with Covid. They have a larger dataset but with weaker correlation between ground truth and reported status of the voice donor, compared to fully clinically validated data. They run SVM and Logistic Regression classifiers with handcrafted spectral features, but the results are unreliable due to the  errors that can be inadvertently or deliberately introduced in the process of self-reporting, as mentioned above.

Other efforts include analyzing selected vowel sounds from speech recordings, e.g counting from 50 to 80, using neural networks, as in the study in  \cite{pinkas2020sars}, which analyzes data collected over cellular phones . It concludes that counting is useful in distinguishing Covid sounds, in particular the /z/ sound. \cite{asiaee2020voice} report results on data collected from clinical settings and descuss how various acoustic parameters of vowel sounds like /aa/ change between the infected and non-infected people. The parameters analyzed include fundamental frequency, jitter and shimmer, HNR etc.

The AI4Covid Application (described in \cite{imran2020ai4covid}) performs the analysis on 70 samples of positive COVID-19 and 96 negative samples and reports 89\% F-1 score for the detection of Covid-19. However, since the data size used is small, the authors do not perform cross-validation experiments.

The study in \cite{pinkas2020sars} performs analysis on 29 positive and 59 negative COVID-19 patient's data with the sounds /ah/, /z/ and also counting, all of which are recorded at the high sampling rate if 32 kHz for all speakers. Their model extracts a feature representation using a transformer RNN network architecture with an added  speaker dissimilarity loss. The final score for their model is obtained using a libSVM based classifier, yielding an AUC of  0.78, obtained with a leave-one-out based cross-validation strategy, owing to the small dataset size.  \cite{bagad2020cough} performs analysis on a relatively large-scale dataset comprising 376 positive cough samples, and 663 negative cough samples. The analysis uses a ResNet-based CNN architecture for making a binary prediction (Covid vs non-COVID) and yields an AUC of 0.68 on their dataset. However, their method uses a relatively high portion (90\%) of the total data for training.


The Coswara dataset \cite{sharma2020coswara} comprises breathing, cough, vocalized sounds, which include the vowels /e/, /i/, /a/, shallow and fast deep breathing sounds collected from  COVID positive and negative patients. They perform  classification using a 9-class classification for the sound categories, with features such as spectral contrast, MFCC, spectral roll-off, zero-crossing rate, spectral bandwidth, spectral flatness etc.,  and achieve an accuracy score of 66.74\% on their test set. The low accuracy presumably stems from the split of the (small amount of) data and from using an unnecessarily high sampling rate (48 kHz) which causes a loss of discriminability in the classification space.

 \cite{10.1145/3394486.3412865} has collected data from 7000 unique users with 235 positive samples only. Features extracted include  standard ones such as duration, tempo, period, RMS, energy, spectral centroid and Vggish based features to generate a 477-dimensional vector from custom features and a 256-dimensional Vggish feature representation. The data collected comprises cough and breath sounds, and the approach yields an AUC of 0.8 for the COVID vs non-COVID classification task.

The research community has yet to work on a dataset with a high number of positive and negative speakers wherein the dataset consists of diverse categories of audio samples which would be an appropriate dataset size to perform k-fold cross-validation with a large-parameter neural network classifier. Our goal in this paper is to find the turning point or cusp where the need for large amounts of data is minimized which the classification accuracy is not compromised. For this, we explore standard less-data intensive classifiers to find the best balance of dataset size, features and classifiers, to achieve our goal.


% according to their paper cough performs the worst and counting is more useful , /z/ sound is also useful as per this paper



% Chloe et.al \cite{brown2020exploring} collect data through voice recordings on a mobile device.

==> expt.backup.tex <==
\section{Data and Experiments} \vspace{-2mm} 
\label{sec:experiments}

\subsection{Dataset and its description}
A key challenge in many of the previous studies was the data -- data that were trustworthy and medically reliable were generally small, while those that were collected at large scale were unreliable (being mostly self-reported) leading to unreliable results.  To address this issue, we require a dataset that is both reasonably large, and reliably annotated.
We used a dataset collected under clinical supervision and curated by Merlin Inc., a private firm in Chile. The subjects usually have symptoms of coughing, sneezing, breathing difficulties etc. So these related symptoms were also recorded along with the voice to account for symptomatic and asymtomatic COVID-19 diagnosis. The COVID positive or negative label was indicated by the subject's lab-certified test results. Additionally metadata also contained information about preexisting conditions such as smoking preference, asthma and detailed comments about the speakers health during the dataset generation. The data samples were recorded over a smartphone, and sampled at 8khz.  

The dataset consists of recordings from 421 covid-positive 989 covid-negative unique subjects. Subjects were asked to record themselves saying the elongated vowels /AH/, /UW/ and /IY/, and speaking the Spanish alphabet (a-z), counting from 1-20 (in Spanish) and producing coughs. 
%The voice recordings of a-z were segmented into vowels of /aaa/ /ee/ /oo/ based on the phonemes. 
To eliminate external influences, subjects were recorded in a quiet room environment.  
%So the dataset has a sampling rate of 8 khz as the microphone bandwidth. 
%The following dataset provides information about the statistics of different metrics in the dataset. 
The total duration of the covid-positive recordings is 17.5 hours, and for covid-negative recordings is 20.5 hours with over 37 hours of total data.

The careful curation of data also enabled us to compile additional statistics that are likely to be relevant to Covid-19. 

Figure \ref{fig:symptoms} shows a chart of symptoms for covid-positive and covid-negative subjects.
\begin{figure}[h]
\centering
\includegraphics[width=8.5cm, height=4cm]{symptoms_0_plot_2.png}
\includegraphics[width=8.5cm, height=4cm]{symptoms_1_plot_2.png}
\caption{The top figures shows the distribution of symptoms in COVID-19 positive patients and the lower figure is the distribution of symptoms in COVID-19 negative individuals (breath-diff stands for breathing difficulty). The rows represents each symptom whereas the column represents the frequency of occurrence of a symptom which are marked by dots}\label{fig:symptoms}
\end{figure}

The occurrence of Covid (and the symptoms arising from it) is also reportedly related to the age and gender of the subjects. Moreover, its symptoms  

\subsection{Experiments}

We perform numerous experiments for the detection of COVID where the input is only the voice signal. In all experiments, the speakers in the training set were separate from those in the test set to ensure that the models do not inadvertently simply capture speaker identity. Thus, we split the data in $k$ fold cross-validation sets based on speaker identity.
%ies by first selecting the speaker and keeping all recordings corresponding to that speaker in the same set. This type of split which is different from research papers published will ensure that there is no bias and we will have an unseen speaker in the testing set due to the experimental design, thereby rendering speaker-id identifying features useless. 

We run various classifiers on our data such as RandomForest (RF), Support Vector Machines (SVMs) with Radial Basis Function and Logistic Regression (LR). We analysed all the spectral features on each of these classifiers including combination of features like Ovec and Custom. The RandomForest runs on $k$ fold equal to 3, 5 and 10. We run grid search on all these classifiers to find the best parameters, particularly experimenting with $\gamma$. We report the performance in the  Section \ref{sec:results}.

\section{Results and Discussion}
\label{sec:results}
From the dataset consisting of a total of 1410 speakers (or 8460 audio recordings), the entire metadata was received for a total of 815 speakers, out of which there were 296 males and 519 females. \vspace{-2mm} 
\subsection{Age based Analysis}
We have broadly categorized the ages into four groups, including the ones whose age was missing, shown in Table \ref{tab:gender_table}.
\begin{itemize}[leftmargin=*] \itemsep0em
    \item Group 1 : age $<=$ 30 years
    \item Group 2 : 30 $<$ age $<=$ 40 years
    \item Group 3 : 40 years $<$ age
    \item Group 4 : Age was missing
\end{itemize}
For patients with age $>$ 40, our classifier is capable of recognizing COVID-19 patients accurately 65\% of the times whereas those with age $<$ 30, classifier is capable of accurately detecting 56\% of the times. 
\begin{table}[h]
    \centering
    \begin{tabular}{|c|c|c|c|c|}
        \hline 
        \textbf{Gender} & \textbf{Group1} & \textbf{Group2} & \textbf{Group3} & \textbf{Group4} \\
        \hline \hline
            Male & 65 & 80 & 80 & 71\\
            Female & 127 & 129 & 145 & 115 \\
            \hline
    \end{tabular}
    \caption{Gender based age analysis}
    \label{tab:gender_table}
        \vspace{-2mm}
\end{table}
The classifier is more reliably able to detect COVID-19 in case of females over males. 
% \begin{figure}[h]
% \centering
% \includegraphics[width=8cm, height=2.5cm]{images/age_dist_0.JPG}
% \includegraphics[width=8cm, height=2.5cm]{images/age_dist_1.JPG}
% \caption{The top figure is the age distribution for Covid positive patients and the lower figure is the age distribution for Covid negative individuals.}
%     \vspace{-2mm}
% \end{figure}





We find Sore-throat is present in most of COVID-19 cases where we are able to detect COVID-19 in 57\% of the cases. When sneeze is present, the classifier is capable of detecting COVID-19 in 47\% of the cases. When cough is a known  symptom for the speaker, then our classifier detects COVID-19 in 73\% of the cases.  \vspace{-2mm} 

\subsection{Smokers and People with Asthma}
Having a previous history of asthma or smoking might put people at a higher risk of COVID \cite{asthma}. We received data where people had a history of asthma and/or were smokers. Table \ref{tab:asthma_table} shows the statistics in our data. Our experimental results indicate asthama is more correlated to COVID-19 than smoking.  
For the patients with COVID-19 and smoking habit, our classifier is accurate by detecting COVID-19 in 66 percent of cases whereas those with COVID-19 and asthama cases we are able to detect COVID-19 accurately in 80 percent of the cases. 

\begin{table}[h]
    \centering
    \begin{tabular}{c|c|c}
        \textbf{Gender} & \textbf{Has Asthma} & \textbf{Is Smoker} \\
        \hline \hline
            Male & 12 & 95\\
            Female & 38 & 139
    \end{tabular}
    \caption{Gender based asthma and smoker statistics}
        \vspace{-4mm}
    \label{tab:asthma_table}
\end{table}


\subsection{Difference in days of diagnosis and data collection }  % \vspace{-2mm} 
The data collection process introduces a delay between the COVID onset and when the voice sample was recorded. Each speaker is labelled for the day they got diagnosed and the day they recorded their data.  Table \ref{tab:diagnosis_table} shows number of people distribution depending on when they were diagnosed (eg. 1 week ago, between 1-2 weeks or greater than 2 weeks) 

\begin{table}[h]
\centering
    \begin{tabular}{ |c|c| } 
         \hline
         \textbf{Diagnosis Day Range} & \textbf{Number of People} \\
         \hline \hline
         Diagnosis day $<=$ 7 days & 95 \\ 
         \hline
         7 days $<$ Diagnosis day $<=$ 14 days & 209 \\ 
         \hline
         Diagnosis day $>$ 14 days & 159 \\ 
         \hline
         Diagnosis day not known & 37 \\
         \hline
    \end{tabular}
    \caption{Difference between Diagnosis Day and Data collection day}
    \vspace{-4mm}
    \label{tab:diagnosis_table}
\end{table}

In general, we find that COVID-19 can be more reliably detected for patients whose voice samples have been collected within 14 days of diagnosis, than for those whose samples were collected after this period.



% For the detection of COVID-19 depending on the amount of diagnosis days, we find that COVID-19 can be reliably detected for patients which are less than 14 days and the degree of correlation for patients with greater than 14 days for diagnosis in the voice samples reduces. 

%Table 1 shows the confusion matrix of the related labels. 


% Confusion matrix


% We split the data into $k$ fold cross validation sets based on the speaker identities to avoid bias and have unseen speaker in the test process in the experimental design. 


%Finally, we use a deep neural network model, in an \textit{autoencoder} architecture using CNN, to extract learned features from the COVID dataset and then use those learned features in an MLP classification network. The details of the model are explained in the Experiment section. 

% Features which are present from pase features. Doesnt have direct correlation with noun capacity. Vocal tract of speech production mechanism 

% Not directly correlated feature in the detection pipeline. 
% Compare the spectrogram, pase and mfcc features --> reason why it is not 

% Randomforest 
% and CNN comparable results as the Randomforest 








% \subsection{Experiments using the different folds}
% We perform K fold cross validation on the dataset. To 
% In order to make full usage of the dataset, we have done the K-folds setting. To do so, we divide the dataset according to the speakers into K-fold for training and testing. The speakers in the test set is not seen in the training set. 
%We perform grid search 


% \section{Results and Discussion}
% 

\begin{table}[h]
    \centering
    \resizebox{1.0\columnwidth}{!}{
    \begin{tabular}{|c|c|c|c|}
    \hline 
       \textbf{Classifier}  &  \textbf{Feature}  & \textbf{AUC} \\ 
       \hline \hline
        Random Forest & Ovec & 0.76 \\
        Random Forest & PANN & 0.78    \\
        Random Forest & vggish & 0.59   \\
        Random Forest & Open-L3 & 0.64   \\
        Random Forest & YAMNet & 0.72   \\
        Random Forest & Custom  Feat & 0.82  \\ 
        Random Forest & Ovec + Custom  Feat & 0.84  \\
        Random Forest & Ovec + Custom Feat + vggish & 0.82  \\
        Random Forest & Ovec + custom feature + YAMNet & 0.86  \\ 
        CNN & Spectrogram & 0.69   \\
        CNN & PASE & 0.73     \\ 
        \hline
    \end{tabular}
    }
    \caption{Results obtained on the full dataset set. Here Ovec refers to features obtained using OpenSMILE, PASE using PASE architecture, custom spectral feature. Random Forest classifier is robust and have improved performance in comparison to CNN based classifier}
    \label{tab:my_label}
        \vspace{-4mm}
\end{table}
\vspace{-2mm} 
\subsection{Audio type analysis}  
% vowel 
We analyze classifier performance according to the audio-type, to identify which type of recording is most suited to capture the voice signatures related to COVID-19. Our results indicate that vowel /IY/ and vowel /UW/ are better at detecting COVID-19 than other types of audio samples. Cough samples are also useful in detecting COVID-19. \vspace{-2mm} 
\subsection{Overall Classifier results} 
Table \ref{tab:my_label} proves our hypothesis that a binary classifier such as Random Forest can perform better for COVID-19 detection than CNN counterparts when faced with limited data. Our experiments have observed that Open-L3 features perform the same as vggish feature representations. Figure \ref{fig:Best} shows the best AUC score achieved of 0.94 and ROC score of 0.85 for the Random forest based classifier with Ovec and custom features on a trimmed down dataset where 20\% samples were heard to contain noise in the recordings. 

\begin{figure}[h]
\centering
\begin{subfigure}[b]{0.23\textwidth}\centering
\includegraphics[width=\textwidth,height=3cm]{roc_auc.png}
\end{subfigure}
\begin{subfigure}[b]{0.23\textwidth}\centering
\includegraphics[width=\textwidth,height=3cm]{prec_recall.png}
\end{subfigure}
 \hspace*{\fill}
\caption{AUC of 0.94 and  ROC of 0.85 is obtained using Random Forest based classifier with Ovec and custom feature vector}
\label{fig:Best}
\end{figure}


\section{Conclusion}
\label{sec:discuss}
Motivated by the urgent need to have alternative methods to augment the medical tests, we designed the experimental setup for the COVID-19 analysis using a wide variety of voice samples. Our analysis provided insights into the type of voice sample which would work best for detecting COVID-19 patients which is the \/eee\/ and \/ooo\/ sounds. Our COVID-19 dataset used in the study was acquired through self-recording using a smartphone application making acquistion feasible at large scale. The preliminary results imply a feasibility for the use of this globally accessible data collection for Sars-COV-2 detection although it doesn't replace RT-PCR or RAT tests.  Our results prove that using a binary classifiers such as Random Forest are more feasible to separate between COVID-19 vs non COVID-19 speakers over data intensive neural network classifiers. We find these binary classifiers to generate better and robust results given the limited amount of data available for analysis. 






%\vfill\pagebreak

% \section{REFERENCES}
% \label{sec:refs}

% List and number all bibliographical references at the end of the
% paper. The references can be numbered in alphabetic order or in
% order of appearance in the document. When referring to them in
% the text, type the corresponding reference number in square
% brackets as shown at the end of this sentence \cite{C2}. An
% additional final page (the fifth page, in most cases) is
% allowed, but must contain only references to the prior
% literature.

% References should be produced using the bibtex program from suitable
% BiBTeX files (here: strings, refs, manuals). The IEEEbib.bst bibliography
% style file from IEEE produces unsorted bibliography list.
% -------------------------------------------------------------------------
\bibliographystyle{IEEEbib}
\bibliography{strings,refs}

==> relatedwork.backup.tex <==
Analysis of vocal sounds has been investigated for the detection of numerous diseases \cite{singh2021overview}. Recently many researchers have developed voice based analyzers for the detection of Covid-19 \cite{9414201_soham,bagad2020cough,schuller2021covid,imran2020ai4covid,despotovic2021detection}. So far, the research has focused on two aspects -- the collection and curation of reliable data in possibly non-clinical settings (e.g. crowsourced settings) and  the determination of which vocal sounds might be most discriminative for the detection of Covid-19. Examples include Chloe et.al \cite{brown2020exploring} who collect cough and breathing samples from people who self-report as being infected with Covid. They have a larger dataset but with weaker correlation between ground truth and reported status of the voice donor, compared to fully clinically validated data. They run SVM and Logistic Regression classifiers with handcrafted spectral features, but the results are unreliable due to the  errors that can be inadvertently or deliberately introduced in the process of self-reporting, as mentioned above.

Other efforts include analyzing selected vowel sounds from speech recordings, e.g counting from 50 to 80, using neural networks, as in the study in  \cite{pinkas2020sars}, which analyzes data collected over cellular phones . It concludes that counting is useful in distinguishing Covid sounds, in particular the /z/ sound. \cite{asiaee2020voice} report results on data collected from clinical settings and descuss how various acoustic parameters of vowel sounds like /aa/ change between the infected and non-infected people. The parameters analyzed include fundamental frequency, jitter and shimmer, HNR etc.

The AI4Covid Application (described in \cite{imran2020ai4covid}) performs the analysis on 70 samples of positive COVID-19 and 96 negative samples and reports 89\% F-1 score for the detection of Covid-19. However, since the data size used is small, the authors do not perform cross-validation experiments.

The study in \cite{pinkas2020sars} performs analysis on 29 positive and 59 negative COVID-19 patient's data with the sounds /ah/, /z/ and also counting, all of which are recorded at the high sampling rate if 32 kHz for all speakers. Their model extracts a feature representation using a transformer RNN network architecture with an added  speaker dissimilarity loss. The final score for their model is obtained using a libSVM based classifier, yielding an AUC of  0.78, obtained with a leave-one-out based cross-validation strategy, owing to the small dataset size.  \cite{bagad2020cough} performs analysis on a relatively large-scale dataset comprising 376 positive cough samples, and 663 negative cough samples. The analysis uses a ResNet-based CNN architecture for making a binary prediction (Covid vs non-COVID) and yields an AUC of 0.68 on their dataset. However, their method uses a relatively high portion (90\%) of the total data for training.


The Coswara dataset \cite{sharma2020coswara} comprises breathing, cough, vocalized sounds, which include the vowels /e/, /i/, /a/, shallow and fast deep breathing sounds collected from  COVID positive and negative patients. They perform  classification using a 9-class classification for the sound categories, with features such as spectral contrast, MFCC, spectral roll-off, zero-crossing rate, spectral bandwidth, spectral flatness etc.,  and achieve an accuracy score of 66.74\% on their test set. The low accuracy presumably stems from the split of the (small amount of) data and from using an unnecessarily high sampling rate (48 kHz) which causes a loss of discriminability in the classification space.

 \cite{10.1145/3394486.3412865} has collected data from 7000 unique users with 235 positive samples only. Features extracted include  standard ones such as duration, tempo, period, RMS, energy, spectral centroid and Vggish based features to generate a 477-dimensional vector from custom features and a 256-dimensional Vggish feature representation. The data collected comprises cough and breath sounds, and the approach yields an AUC of 0.8 for the COVID vs non-COVID classification task.

The research community has yet to work on a dataset with a high number of positive and negative speakers wherein the dataset consists of diverse categories of audio samples which would be an appropriate dataset size to perform k-fold cross-validation with a large-parameter neural network classifier. Our goal in this paper is to find the turning point or cusp where the need for large amounts of data is minimized which the classification accuracy is not compromised. For this, we explore standard less-data intensive classifiers to find the best balance of dataset size, features and classifiers, to achieve our goal.


% according to their paper cough performs the worst and counting is more useful , /z/ sound is also useful as per this paper



% Chloe et.al \cite{brown2020exploring} collect data through voice recordings on a mobile device.
